Modeling human visual search: A combined Bayesian searcher and saliency map approach for eye movement guidance in natural scenes

Finding objects is essential for almost any daily-life visual task. Saliency models have been useful to predict fixation locations in natural images, but are static, i.e., they provide no information about the time-sequence of fixations. Nowadays, one of the biggest challenges in the field is to go beyond saliency maps to predict a sequence of fixations related to a visual task, such as searching for a given target. Bayesian observer models have been proposed for this task, as they represent visual search as an active sampling process. Nevertheless, they were mostly evaluated on artificial images, and how they adapt to natural images remains largely unexplored. Here, we propose a unified Bayesian model for visual search guided by saliency maps as prior information. We validated our model with a visual search experiment in natural scenes recording eye movements. We show that, although state-of-the-art saliency models perform well in predicting the first two fixations in a visual search task, their performance degrades to chance afterward. This suggests that saliency maps alone are good to model bottom-up first impressions, but are not enough to explain the scanpaths when top-down task information is critical. Thus, we propose to use them as priors of Bayesian searchers. This approach leads to a behavior very similar to humans for the whole scanpath, both in the percentage of target found as a function of the fixation rank and the scanpath similarity, reproducing the entire sequence of eye movements.

==> 0_introduction.tex <==
\section{Introduction}
Visual search is a natural task that humans perform in everyday life, from looking for someone in a photograph to searching where you left your favorite mug in the kitchen. Finding our goal relies on our ability to gather visual information through a sequence of eye movements, performing a discrete sampling of the scene. The fixations of the gaze follow different strategies, trying to minimize the number of steps needed to find the target \citep{borji2014defending,rolfs2015attention, tatler2010yarbus, yarbus1967eye}. This process is an example of the active sensing, \jk{as humans perform decisions about future steps making inferences based the information gathered so far to fulfill a task \citep{yang2016theoretical,gottlieb2018towards}}.\commenttex{This way, each decision is expected to reduce uncertainty about the environment \citep{gottlieb2018towards,najemnik2005optimal}.} Moreover, this decision-making behavior depends on the purpose; for instance, whether it is task-driven or simple curiosity. Predicting the eye movements necessary to meet a goal is a computationally-complex task: it must combine the bottom-up information capturing processes and the top-down integration of information and updating of expectations in each fixation.

A related task is the prediction of the most likely fixation positions in the scene to build a \textit{saliency map}, identifying regions that draw our attention within an image \citep{itti2001computational}.\commenttex{The first saliency models were built based on computer vision strategies, combining different filters over the image \citep{itti2001computational}. Some of these filters could be very general, such as a low-pass filter that gives the idea of the horizon \citep{itti1998model, torralba2001statistical}, or more specific, such as detecting high-level features like faces \citep{cerf2008predicting}. In recent years, deep neural networks (DNNs) have advanced the development of saliency maps. Many saliency models have successfully incorporated pre-trained convolutional DNNs in order to extract low and high-level features of the images \citep{kummerer2017understanding,cornia2016deep,cornia2018predicting}. These novel approaches were summarized in MIT/Tuebingen's collaboration website \citep{mit-tuebingen-saliency-benchmark}.} 
Nevertheless, they produce accurate results only in the first few fixations of free exploration tasks \citep{torralba2006contextual} as they cannot make use of the sequential nature of the task nor combine information through the sequence of fixations. Thus, they may not be able to replicate these results when performing a complex task, like visual search. 

Nowadays, there is a growing interest in Bayesian models given their good results at modeling human behavior, and also for having straightforward interpretations related to human information processing \citep{ullman2019using}. For instance, different Bayesian Models were applied to decision making or perceptual tasks \citep{oreilly2012how, rohe2015cortical, samad2015perception, wiecki2015model, turgeon2016cognitive,knill2004bayesian,tenenbaum2006theory, meyniel2015confidence}. In the case of visual search, \citet{najemnik2005optimal} have proposed a model that decides the next eye movement based on its prior knowledge, a visibility map, and the current state of a posterior probability that is updated after every fixation. The results of this Ideal Bayesian searcher (IBS) have had a wide impact, but the images they used in their experiments were all artificial. In order to extend these results to natural images, it is necessary to incorporate the information available in the scene. \commenttex{Recently, \citet{zhang2018finding} explore visual search in natural images with a model based on DNNs, elaborating an attention map related to the search goal. Also, \citet{hoppe2019multi} proposed a model that incorporates planning. It uses the uncertainty of the current observation to select the upcoming gaze locations in order to maximize the probability of detecting the location of the target after the sequence of two saccades. Their task is specifically designed for maximizing the difference between models, i.e finding the target in few fixations on artificial stimuli.}\meledit{Recently, there have been works exploring visual search, but they have used greedy algorithms \citep{zhang2018finding} or only explored the first few fixations on artificial stimuli \citep{hoppe2019multi}.}

Here, we show that an IBS model combined with state-of-the-art saliency maps as priors performs as well as humans in a visual search task on natural scenes images. Moreover, we incorporate a different update rule to the IBS model, based on a correlation for the template response. This modification could incorporate the effect of distractors, even though we did not specifically test this hypothesis. Previous work compares the general performance between humans and models (targets found and total number of fixations). Moving one step further, we quantitatively compare the scanpaths (ordered sequence of fixations) produced by the model with the ones recorded by human observers.


==> modelo_neurips.tex <==

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.

The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.

For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.

Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.

\section{Headings: first level}
\label{headings}

All headings should be lower case (except for first word and proper nouns),
flush left, and bold.

First-level headings should be in 12-point type.

\subsection{Headings: second level}

Second-level headings should be in 10-point type.

\subsubsection{Headings: third level}

Third-level headings should be in 10-point type.

\paragraph{Paragraphs}

There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone.

\subsection{Citations within the text}

The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.

The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}

If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2020+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}

If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2020}
\end{verbatim}

As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''

\subsection{Footnotes}

Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).

Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}

\subsection{Figures}

\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}

All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.

You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.

\subsection{Tables}

All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.

Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.

Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.

\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}

\section{Final instructions}

Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PDF files}

Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''

Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.

\begin{itemize}

\item You should directly generate PDF files using \verb+pdflatex+.

\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.

\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}

\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.

\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.

\end{itemize}

If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.

\subsection{Margins in \LaTeX{}}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})

A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\section*{Broader Impact}

Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
biases in the data. If authors believe this is not applicable to them, authors can simply state this.

Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments go at the end of the paper before the list of references. Moreover, you are required to declare 
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

\section*{References}

References follow the acknowledgments. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
{\bf Note that the Reference section does not count towards the eight pages of content that are allowed.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
(eds.), {\it Advances in Neural Information Processing Systems 7},
pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
  Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
recall at excitatory recurrent synapses and cholinergic modulation in rat
hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.


==> table1-v2.tex <==
\begin{table}[]
\centering
\caption{\textbf{Different measures on performance and scanpath similarity between humans and models}. \textit{Weighted distance} is the distance between humans and model performance weighted by humans dispersion. \textit{Mean Agreement} and \textit{Jaccard Index} measures coincidence of humans and model's correct target detections. \textit{Spearman correlation} quantifies the correlation between humans and model's scanpath similarities. \textit{Linear Regression} corresponds to the slope in a simple $y\sim x$ model, between humans and models. Only correct trials were considered and averaged for each image ($N = 134$). DG2 refers to DeepGaze2.}
\begin{comment}
    \resizebox{0.85\textwidth}{!}{\begin{tabular}{@{}lrrrrrrr@{}}
    \cmidrule(r){1-8} 
    % Primera fila
    \multicolumn{1}{c}{}                                            &
    \multicolumn{3}{c}{\textbf{\{Searcher Model\} + DeepGaze 2}}    &  
    \multicolumn{3}{c}{\textbf{cIBS + \{Saliency Map Prior\}}}      &
    \multicolumn{1}{c}{} \\
    \cmidrule(r){1-8}
      \multicolumn{1}{c}{} &
      \multicolumn{1}{c}{\textbf{IBS}} &
      \multicolumn{1}{c}{\textbf{Greedy}} &
      \multicolumn{1}{c}{\textbf{Saliency}} &
      \multicolumn{1}{c}{\textbf{Center}} &
      \multicolumn{1}{c}{\textbf{Flat}} &
      \multicolumn{1}{c}{\textbf{Noisy}} &
      \multicolumn{1}{c}{\textbf{cIBS + DG2}} \\ \cmidrule(r){1-8}
    Weighted Distance & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
    Mean Agreement & 1 & 1 & 1 & 1 & 1 & 1 & 1\\ 
    Jaccard Index & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
    Linear Regression (Slope) & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
    Spearman Corr & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
    \cmidrule(r){1-8}
    \end{tabular}}
\end{comment}
\resizebox{0.85\textwidth}{!}{\begin{tabular}{@{}lrrrrrrr@{}}
\cmidrule(r){1-8} 
% Primera fila
  \multicolumn{1}{l}{Searcher:} &
  \multicolumn{1}{c}{\textbf{cIBS}} &
  \multicolumn{1}{c}{\textbf{IBS}} &
  \multicolumn{1}{c}{\textbf{Greedy}} &
  \multicolumn{1}{c}{\textbf{Saliency}} &
  \multicolumn{1}{c}{\textbf{cIBS}} &
  \multicolumn{1}{c}{\textbf{cIBS}} &
  \multicolumn{1}{c}{\textbf{cIBS}}\\ 
\cmidrule(r){1-8}
  \multicolumn{1}{l}{Prior:} &
  \multicolumn{1}{c}{\textbf{DG2}} &
  \multicolumn{1}{c}{\textbf{DG2}} &
  \multicolumn{1}{c}{\textbf{DG2}} &
  \multicolumn{1}{c}{\textbf{DG2}} &
  \multicolumn{1}{c}{\textbf{Center}} &
  \multicolumn{1}{c}{\textbf{Flat}} &
  \multicolumn{1}{c}{\textbf{Noisy}}\\ 
\cmidrule(r){1-8}
Weighted Distance & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
Mean Agreement & 1 & 1 & 1 & 1 & 1 & 1 & 1\\ 
Jaccard Index & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
Linear Regression (Slope) & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
Spearman Correlation & 1 & 1 & 1 & 1 & 1 & 1 & 1\\
\cmidrule(r){1-8}
\end{tabular}}
\vspace{-10mm}
\end{table}

==> table1.tex <==

\begin{table}[]
\caption{\jk{NO QUISE DARLO VUELTA... PERO SE PODRIAN PONER LAS METRICAS EN FILAS Y LOS MODELOS EN COLUMNAS. ASÍ LA MAYORIA PUEDE QUEDAR EN UNA SOLA LINEA. Y ADEMAS EL cIBS+DeepGaze2 PUEDE ESTAR UNA SOLA VEZ.} \textbf{Different measures on performance and mean scanpath similarity between humans and mean scanpath similarity between each human and a model observer}. Only correct trials were considered and averaged for each image ($N = 134$).
}
\resizebox{\textwidth}{!}{\begin{tabular}{@{}lrrrrrllrrrrr@{}}
\cmidrule(r){1-6} \cmidrule(l){8-13}
\multicolumn{6}{c}{\textbf{\{Searcher Model\} + DeepGaze 2}}              & \multicolumn{1}{c}{} & \multicolumn{6}{c}{\textbf{cIBS + \{Saliency Map Prior\}}}            \\
\cmidrule(r){1-6} \cmidrule(l){8-13} &
  \multicolumn{1}{c}{ \begin{tabular}[c]{@{}c@{}} Weighted \\ distance\\ between \\ humans\\ and models\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Jaccard\\ Index\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Spearman\\ Correlation\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Linear\\ regression\\ (slope)\\ y $\sim$x1\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Mean\\ agreement\end{tabular}} &
   &
   &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Weighted \\ distance\\ between \\ humans\\ and models\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Jaccard\\ Index\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Spearman\\ Correlation\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Linear\\ regression\\ (slope)\\ y $\sim$x1\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Mean\\ agreement\end{tabular}} \\ \cmidrule(r){1-6} \cmidrule(l){8-13} 
cIBS           & 0,31 & 0,51 (0,098) & 0,50 & 0,84 & 0.64 (0,08) &                      & DeepGaze 2 & 0,31 & 0,51 (0,098) & 0,50 & 0,84 & 0.64 (0,08) \\
IBS            & 0,78 & 0,54 (0,105) & 0,48 & 0,85 & 0.64 (0.09) &                      & Center     & 1,38 & 0,38 (0,086) & 0,50 & 0,88 & 0.59 (0.08) \\
Greedy         & 0,13 & 0,47 (0,091) & 0,44 & 0,76 & 0.62 (0.08) &                      & Flat       & 0,72 & 0,51 (0,109) & 0,54 & 0,69 & 0.60 (0.10) \\
Saliency based & 2,14 & 0,32 (0,073) & 0,22 & 0,52 & 0.55 (0.09) &                      & Noisy      & 0,15 & 0,46 (0,089) & 0,43 & 0,61 & 0.61 (0.08) \\ \cmidrule(r){1-6} \cmidrule(l){8-13} 
\end{tabular}}
\label{table1:metrics}
\end{table}
